Dual constraints with ALMA: new [O III] 88 ${\rm \mu}$m and dust-continuum observations reveal the ISM conditions of luminous LBGs at $z \sim 7$

We present new [O III] 88 ${\rm \mu}$m observations of five bright $z \sim 7$ Lyman-break galaxies spectroscopically confirmed by ALMA through the [C II] 158 ${\rm \mu}$m line, unlike recent [O III] detections where Lyman-${\rm \alpha}$ was used. This nearly doubles the sample of Epoch of Reionisation galaxies with robust ($5 \sigma$) detections of [C II] and [O III]. We perform a multi-wavelength comparison with new deep HST images of the rest-frame UV, whose compact morphology aligns well with [O III] tracing ionised gas. By contrast, we find more spatially extended [C II] emission likely produced in neutral gas, as indicated by a [N II] 205 ${\rm \mu}$m non-detection in one source. We find a positive correlation between the equivalent width of the optical [O III] and H${\rm \beta}$ lines and the [O III]/[C II] ratio, as seen in local metal-poor dwarf galaxies. Cloudy models of a nebula of typical density harbouring a young stellar population with a high ionisation parameter appear to adequately reproduce the far-infrared lines. Surprisingly, however, our models fail to reproduce the strength of [O III] 88 ${\rm \mu}$m, unless we assume an ${\rm \alpha}$/Fe enhancement and a near-solar nebular oxygen abundance. On spatially resolved scales, we find [O III]/[C II] shows a tentative anti-correlation with infrared excess, $L_{\rm IR}/L_{\rm UV}$, also seen on global scales in the local Universe. Finally, we introduce the far-infrared spectral energy distribution fitting code MERCURIUS to show that dust-continuum measurements of one source appear to favour a low dust temperature coupled with a high dust mass. This implies a high stellar metallicity yield and may point towards the need of dust production or grain-growth mechanisms beyond supernovae.

==> ALMA OIII CII/ALMA_cont_fluxes.tex <==
Regime & Quantity & \setulcolor{COS2987}\ul{COS-2987030247} & \setulcolor{COS3018}\ul{COS-3018555981} & \setulcolor{UVIS001}\ul{UVISTA-Z-001} & \setulcolor{UVIS007}\ul{UVISTA-Z-007} & \setulcolor{UVIS019}\ul{UVISTA-Z-019}
\\
\hline
\multirow{4}{*}{Band 8} & $\nu_\text{obs} \, (\mathrm{GHz})$ & $426.2_{ -6.7 }^{ +9.3 }$ & $422.5_{ -5.4 }^{ +8.4 }$ & $413.0_{ -6.9 }^{ +8.9 }$ & $434.5_{ -7.7 }^{ +6.2 }$ & $434.4_{ -7.8 }^{ +6.1 }$
\\
& $\lambda_\text{{emit}} \, (\mathrm{{\upmu m}})$ & $90.1_{ -1.9 }^{ +1.4 }$ & $90.3_{ -1.8 }^{ +1.2 }$ & $90.0_{ -1.9 }^{ +1.5 }$ & $89.0_{ -1.3 }^{ +1.6 }$ & $89.0_{ -1.2 }^{ +1.6 }$
\\
& $S_{\nu\text{, obs}} \, (\mathrm{\upmu Jy})$ & $<163 \, (160)$ & $<210 \, (240)$ & $189 \pm 100$ & $<361 \, (260)$ & $<840 \, (625)$
\\
\vspace{1.5ex}
& $A_\text{dust} \, (\mathrm{kpc^2})$ & \dots & \dots & $(5.2 \pm 2.4) \times$ \newline $(2.0 \pm 1.3)$ & \dots & \dots
\\
\multirow{4}{*}{Band 6} & $\nu_\text{obs} \, (\mathrm{GHz})$ & $250.3_{ -9.8 }^{ +7.3 }$ & $232.1_{ -8.0 }^{ +13.3 }$ & $232.9_{ -16.0 }^{ +10.0 }$ & $242.4_{ -2.1 }^{ +2.0 }$ & $237.3_{ -11.0 }^{ +8.8 }$
\\
& $\lambda_\text{{emit}} \, (\mathrm{{\upmu m}})$ & $153.4_{ -4.4 }^{ +6.2 }$ & $164.5_{ -8.9 }^{ +5.9 }$ & $159.6_{ -6.6 }^{ +11.8 }$ & $159.6_{ -1.3 }^{ +1.4 }$ & $162.9_{ -5.8 }^{ +7.9 }$
\\
& $S_{\nu\text{, obs}} \, (\mathrm{\upmu Jy})$ & $<22.5 \, (18.4)$ & $76 \pm 13$ & $97 \pm 30$ & $<69.6 \, (81.8)$ & $131 \pm 36$
\\
\vspace{1.5ex}
& $A_\text{dust} \, (\mathrm{kpc^2})$ & \dots & $(4.3 \pm 0.8) \times$ \newline $(3.6 \pm 0.7)$ & $(10.3 \pm 3.4) \times$ \newline $(3.7 \pm 3.0)$ & \dots & $(4.1 \pm 1.1) \times$ \newline $(3.0 \pm 0.9)$
\\
\multirow{3}{*}{Band 5} & $\nu_\text{obs} \, (\mathrm{GHz})$ & $195.6_{ -9.4 }^{ +6.4 }$ & \dots & \dots & \dots & \dots
\\
& $\lambda_\text{{emit}} \, (\mathrm{{\upmu m}})$ & $196.3_{ -6.3 }^{ +9.9 }$ & \dots & \dots & \dots & \dots
\\
& $S_{\nu\text{, obs}} \, (\mathrm{\upmu Jy})$ & $<19.4 \, (22.8)$ & \dots & \dots & \dots & \dots
\\
&  &  &  &  &  & 
\\
\cline{2-7}
& $T_\text{dust}$ & Fixed: $50 \, \mathrm{K}$ & \glsentryshort{MERCURIUS} fit & \glsentryshort{MERCURIUS} fit & Fixed: $50 \, \mathrm{K}$ & \glsentryshort{MERCURIUS} fit
\\
& $\lambda_0$ (opacity) & Optically thin & Self-consistent: $8.4_{ -4.4 }^{ +11.8 } \, \mathrm{ \upmu m }$ & Self-consistent: $0.6_{ -0.3 }^{ +0.7 } \, \mathrm{ \upmu m }$ & Optically thin & Self-consistent: $4.2_{ -2.7 }^{ +7.5 } \, \mathrm{ \upmu m }$
\\
& $\beta_\text{\gls{IR}}$ & Fixed: $1.5$ & Fixed: $1.5$ & Fixed: $1.5$ & Fixed: $1.5$ & Fixed: $1.5$
\\
\cline{2-7}
&  &  &  &  &  & 
\\
& $M_\text{dust} \, (\mathrm{M_\odot})$ & $\lesssim4 \cdot 10^{6}$ & $7_{-5}^{+19} \cdot 10^{7}$ & $4_{-3}^{+8} \cdot 10^{6}$ & $\lesssim1 \cdot 10^{7}$ & $2.1_{-1.6}^{+7.6} \cdot 10^{7}$
\\
& $\Sigma_\text{dust} \, (\mathrm{M_\odot \, pc^{-2}})$ & \dots & $7_{-4}^{+18}$ & $0.1_{-0.1}^{+0.3}$ & \dots & $2.3_{-1.8}^{+8.5}$
\\
& $M_\text{dust} / M_*$ & $\lesssim0.002$ & $0.05_{-0.04}^{+0.16}$ & $0.001_{-0.0007}^{+0.003}$ & $\lesssim0.003$ & $0.007_{-0.006}^{+0.03}$
\\
& $y_\text{dust, AGB} \, (\mathrm{M_\odot})$ & $\lesssim0.1$ & $1.5_{-1.1}^{+4.6}$ & $0.03_{-0.02}^{+0.08}$ & $\lesssim0.1$ & $0.2_{-0.2}^{+0.9}$
\\
\vspace{1.5ex}
& $y_\text{dust, SN} \, (\mathrm{M_\odot})$ & $\lesssim0.2$ & $4.5_{-3.1}^{+13.3}$ & $0.09_{-0.06}^{+0.2}$ & $\lesssim0.3$ & $0.6_{-0.5}^{+2}$
\\
& $T_\text{dust} \, (\mathrm{K})$ & \dots & $29_{-5}^{+9}$ ($<48$) & $59_{-20}^{+41}$ & \dots & $47_{-17}^{+40}$
\\
\vspace{1.5ex}
& $T_\text{peak} \, (\mathrm{K})$ & \dots & $26_{-5}^{+8}$ ($<43$) & $53_{-17}^{+37}$ & \dots & $42_{-15}^{+35}$
\\
$8$-$1000 \, \mathrm{\upmu m}$ & $L_\mathrm{IR} \, (\mathrm{L_\odot})$ & $\lesssim2.1 \cdot 10^{11}$ & $9.9_{-2.3}^{+6.8} \cdot 10^{10}$ & $2.0_{-1.3}^{+9.5} \cdot 10^{11}$ & $\lesssim6.9 \cdot 10^{11}$ & $3.1_{-1.8}^{+18.1} \cdot 10^{11}$
\\
\vspace{1.5ex}
$42.5$-$122.5 \, \mathrm{\upmu m}$ & $L_\mathrm{FIR} \, (\mathrm{L_\odot})$ & $\lesssim1.4 \cdot 10^{11}$ & $6.4_{-1.6}^{+4.8} \cdot 10^{10}$ & $1.1_{-0.6}^{+1.1} \cdot 10^{11}$ & $\lesssim4.7 \cdot 10^{11}$ & $2.1_{-1.3}^{+4.2} \cdot 10^{11}$
\\
$\mathrm{IR}$ ($8$-$1000 \, \mathrm{\upmu m}$) & $\text{SFR}_\text{IR} \, (\mathrm{M_\odot \, yr^{-1}})$ & $\lesssim32$ & $15_{-3}^{+10}$ & $30_{-20}^{+142}$ & $\lesssim102$ & $46_{-27}^{+270}$
\\
$\mathrm{UV+IR}$ & $\text{SFR}_\text{tot} \, (\mathrm{M_\odot \, yr^{-1}})$ & $\lesssim54$ & $34_{-4}^{+10}$ & $79_{-20}^{+142}$ & $\lesssim128$ & $63_{-27}^{+270}$
\\
